Encoding Invariances in Deep Generative Models

Reliable training of generative adversarial networks (GANs) typically require massive datasets in order to model complicated distributions. However, in several applications, training samples obey invariances that are \textit{a priori} known; for example, in complex physics simulations, the training data obey universal laws encoded as well-defined mathematical equations. In this paper, we propose a new generative modeling approach, InvNet, that can efficiently model data spaces with known invariances. We devise an adversarial training algorithm to encode them into data distribution. We validate our framework in three experimental settings: generating images with fixed motifs; solving nonlinear partial differential equations (PDEs); and reconstructing two-phase microstructures with desired statistical properties. We complement our experiments with several theoretical results.

==> invnet_dia.tex <==
%% Creator: Inkscape inkscape 0.92.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'fig/invnet.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{603.58929972bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.71019816)%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{fig/invnet.pdf}}%
    \put(0.05821788,0.26015051){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{z}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{fig/invnet.pdf}}%
    \put(0.02155524,0.25958673){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{d}}}%
    \put(0.16963938,0.25981854){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{G(.)}}}%
    \put(0.27321322,0.49023105){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{fig/invnet.pdf}}%
    \put(0.45214554,0.49092976){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{D(.)}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{fig/invnet.pdf}}%
    \put(0.57194253,0.47808791){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{fake}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{fig/invnet.pdf}}%
    \put(0.57504241,0.50992862){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{real}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=6]{fig/invnet.pdf}}%
    \put(0.45212004,0.1260377){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{I(.)}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=7]{fig/invnet.pdf}}%
    \put(0.54386975,0.09984764){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{Compare}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=8]{fig/invnet.pdf}}%
    \put(0.79330486,0.45098192){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=9]{fig/invnet.pdf}}%
    \put(0.87313042,0.29717481){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{+}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=10]{fig/invnet.pdf}}%
    \put(0.94863162,0.19400166){\color[rgb]{1,1,1}\makebox(0,0)[lb]{\smash{\textbf{+}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=11]{fig/invnet.pdf}}%
    \put(0.60880909,0.16083506){\color[rgb]{1,1,1}\makebox(0,0)[lb]{\smash{\textbf{+}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=12]{fig/invnet.pdf}}%
    \put(0.87022805,0.29888791){\color[rgb]{1,1,1}\makebox(0,0)[lb]{\smash{\textbf{+}}}}%
    \put(0.70697274,0.66609781){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.37369069\unitlength}\raggedright Training through \\ Back-propagation\end{minipage}}}%
    \put(0.21596002,0.51411615){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.12042062\unitlength}\centering \scriptsize{Real\\ Images \\ from\\ MNIST data}\end{minipage}}}%
    \put(0.67808642,0.25650126){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.20679863\unitlength}\centering \small{Invariance :\\ enforces the motif\\ on generated image}\end{minipage}}}%
    \put(0.61017014,0.36222564){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.20679863\unitlength}\centering \small{Generator :\\ learns MNIST digits \\ with motifs}\end{minipage}}}%
    \put(0.69001962,0.46746331){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\begin{minipage}{0.20679863\unitlength}\centering \small{Discriminator :\\ learns and enforces\\ MNIST digits}\end{minipage}}}%
  \end{picture}%
\endgroup%

